LITE: LLM-Impelled efficient Taxonomy Evaluation

This paper presents LITE, an LLM-based evaluation method designed for efficient and flexible assessment of taxonomy quality. To address challenges in large-scale taxonomy evaluation, such as efficiency, fairness, and consistency, LITE adopts a top-down hierarchical evaluation strategy, breaking down the taxonomy into manageable substructures and ensuring result reliability through cross-validation and standardized input formats. LITE also introduces a penalty mechanism to handle extreme cases and provides both quantitative performance analysis and qualitative insights by integrating evaluation metrics closely aligned with task objectives. Experimental results show that LITE demonstrates high reliability in complex evaluation tasks, effectively identifying semantic errors, logical contradictions, and structural flaws in taxonomies, while offering directions for improvement. Code is available at https://github.com/Zhang-l-i-n/TAXONOMY_DETECT .

==> latex/sections/00.Introduction.00.tex <==
% - Taxonomy的重要性  
% - 不同领域和业务需求推动了多种版本的Taxonomy开发及迭代。 
Taxonomies play a crucial role in structuring knowledge, enhancing information retrieval, and supporting task understanding through hierarchical relationships among concepts\cite{Welty2001Supporting, 10.1145/3289600.3290972}.
However, they vary significantly across different applications and domains, each requiring tailored structures to meet specific needs\cite{Glass1995Contemporary,Bordea2020Evaluation}. 
Additionally, taxonomies undergo evolution as they must be updated and refined to incorporate new knowledge and correct past inconsistencies. 
This variability and continuous evolution pose significant challenges in assessing taxonomy quality, making evaluation both essential and complex\cite{Jabborov2023Taxonomy,Degrossi2018A,Alers-García2021Resources}.

% - 评估的挑战 以及 当前方法局限   
As taxonomies evolve, an effective evaluation framework is essential for their improvement. 
However, current methods have several limitations. 
There is no universal standard for different domains, and most approaches focus on structural alignment using traditional metrics like statistical consistency, which fail to capture the semantic and contextual relevance of taxonomies in real-world settings\cite{Jiang2022TaxoEnrich:,Carrion2019A,Liu2024An}. This makes it difficult to assess how well a taxonomy meets practical requirements. 
Additionally, current methods struggle with the complexity of domain knowledge and business language, limiting their real-world applicability. An ideal approach should combine quantitative metrics with qualitative insights to identify weaknesses and guide improvements, enabling effective refinement based on actual needs\cite{Kumar2022K-LM,McDaniel2019Evaluating}.

% - 提出用LLM评估，LLM的潜在优势，为什么选择LLM  
To address these challenges, we propose using large language models (LLMs) for Taxonomy evaluation. 
LLMs are highly effective in natural language understanding and generation, enabling them to assess Taxonomies across various domains\cite{Raiaan2024A}. Their ability to understand complex business language allows for a deeper evaluation of how Taxonomies align with real-world objectives. 
By integrating LLMs, we aim to bridge the gap between traditional structural evaluation and the nuanced needs of practical applications, making the evaluation more context-aware and adaptable. 
Additionally, LLMs can offer insights for improvements, enhancing both accuracy and relevance\cite{Upadhyay2024LLMs}.

% - 研究贡献 
%   - 提出了一种基于LLM的Taxonomy评估方法，弥补现有方法的不足。  
%   - 针对大规模Taxonomy设计评估方法，使方法有效且高效。
%   - 设计了与业务目标对齐的评估指标，综合量化与定性分析。  
%   - 通过构建LLM驱动的评估方法，提升Taxonomy质量评估的科学性和实用性，为未来的Taxonomy设计和迭代提供支持。
However, applying LLMs for large-scale Taxonomy evaluation introduces several challenges. 
First, efficiency is a major concern,  as evaluating large Taxonomies with hundreds of thousands of nodes can be computationally heavy, making the process slow and costly. 
Second, maintaining fairness and consistency in LLM-based evaluation is difficult, as repeated queries may lead to scoring variations or biases across different hierarchical structures\cite{Gallegos2023Bias}. 
Additionally, current evaluation methods often focus too much on numerical evaluation and overlook qualitative insights, which are essential for improving Taxonomy structures based on real-world usage.

To address these challenges, we propose \textbf{L}LM-\textbf{I}mpelled \textbf{T}axonomy \textbf{E}valuation for Efficiency(\textbf{\methode}). 
Our approach incorporates a top-down hierarchical evaluation strategy, partitioning Taxonomies into manageable substructures to enhance evaluation efficiency. 
Additionally, we introduce penalty mechanisms to mitigate extreme scoring variations, ensuring fairness and reliability across different Taxonomy levels. 
Most importantly, \methode~integrates evaluation metrics that align closely with task-oriented objectives, enabling both quantitative performance analysis and qualitative insights into semantic and structural coherence. 
Through these approaches, \methode~systematically identifies weaknesses in Taxonomies and provides actionable recommendations for optimization and iteration.


By introducing this LLM-driven evaluation framework, we improve the accuracy and practical use of taxonomy quality evaluation.
Our experimental results demonstrate the defects of taxonomies under different construction methods (shown in Sec.\ref{ana:taxo}), showcasing the effectiveness of \methode~in advancing Taxonomy evaluation and refinement.


==> latex/sections/00.Introduction.01.tex <==
Taxonomies play a crucial role in structuring knowledge, enhancing information retrieval, and supporting task understanding through hierarchical relationships among concepts\cite{Welty2001Supporting, 10.1145/3289600.3290972}.
However, they vary significantly across different applications and domains, each requiring tailored structures to meet specific needs\cite{Glass1995Contemporary,Bordea2020Evaluation}. 
Additionally, taxonomies undergo evolution as they must be updated and refined to incorporate new knowledge and correct past inconsistencies. 
This variability and continuous evolution pose significant challenges in assessing taxonomy quality, making evaluation both essential and complex\cite{Jabborov2023Taxonomy,Degrossi2018A,Alers-García2021Resources}.

As taxonomies evolve, an effective evaluation framework is essential for their improvement. 
However, current methods have several limitations. 
There is no universal standard for different domains, and most approaches focus on structural alignment using traditional metrics like statistical consistency, which fail to capture the semantic and contextual relevance of taxonomies in real-world settings\cite{Jiang2022TaxoEnrich:,Carrion2019A,Liu2024An}. This makes it difficult to assess how well a taxonomy meets practical requirements. 
Additionally, current methods struggle with the complexity of domain knowledge and business language, limiting their real-world applicability. An ideal approach should combine quantitative metrics with qualitative insights to identify weaknesses and guide improvements, enabling effective refinement based on actual needs\cite{Kumar2022K-LM,McDaniel2019Evaluating}.

To address these challenges, we propose using large language models (LLMs) for Taxonomy evaluation. 
LLMs are highly effective in natural language understanding and generation, enabling them to assess Taxonomies across various domains\cite{Raiaan2024A}. Their ability to understand complex business language allows for a deeper evaluation of how Taxonomies align with real-world objectives. 
By integrating LLMs, we aim to bridge the gap between traditional structural evaluation and the nuanced needs of practical applications, making the evaluation more context-aware and adaptable. 
Additionally, LLMs can offer insights for improvements, enhancing both accuracy and relevance\cite{Upadhyay2024LLMs}.

However, applying LLMs for large-scale Taxonomy evaluation introduces several challenges. 
First, efficiency is a major concern,  as evaluating large Taxonomies with hundreds of thousands of nodes can be computationally heavy, making the process slow and costly. 
Second, maintaining fairness and consistency in LLM-based evaluation is difficult, as repeated queries may lead to scoring variations or biases across different hierarchical structures\cite{Gallegos2023Bias}. 
Additionally, current evaluation methods often focus too much on numerical evaluation and overlook qualitative insights, which are essential for improving Taxonomy structures based on real-world usage.

To address these challenges, we propose \textbf{L}LM-\textbf{I}mpelled \textbf{T}axonomy \textbf{E}valuation for Efficiency(\textbf{\methode}). 
Our approach incorporates a top-down hierarchical evaluation strategy, partitioning Taxonomies into manageable substructures to enhance evaluation efficiency. 
Additionally, we introduce penalty mechanisms to mitigate extreme scoring variations, ensuring fairness and reliability across different Taxonomy levels. 
Most importantly, \methode~integrates evaluation metrics that align closely with task-oriented objectives, enabling both quantitative performance analysis and qualitative insights into semantic and structural coherence. 
Through these approaches, \methode~systematically identifies weaknesses in Taxonomies and provides actionable recommendations for optimization and iteration.


By introducing this LLM-driven evaluation framework, we improve the accuracy and practical use of taxonomy quality evaluation.
Our experimental results demonstrate the defects of taxonomies under different construction methods (shown in Sec.\ref{ana:taxo}), showcasing the effectiveness of \methode~in advancing Taxonomy evaluation and refinement.

Taxonomy在知识组织、信息检索和任务理解等领域扮演着关键角色，主要通过建立概念间的层级关系来实现这些功能\cite{Welty2001Supporting, 10.1145/3289600.3290972}。
然而，不同应用领域和场景对taxonomy的结构和内容要求各异，这种多样性使得taxonomy的构建和评估面临重大挑战\cite{Glass1995Contemporary,Bordea2020Evaluation}。
尽管taxonomy的评估对其质量保证和持续优化至关重要，但现有的评估方法存在明显局限性，难以满足实际应用需求。

传统的taxonomy评估方法主要分为两类：
一类聚焦局部上下位关系的合理性~\cite{Jiang2022TaxoEnrich:, shen2020taxoexpan,gu2023gantee,cheng2022learning}，另一类则聚焦于taxonomy的整体结构\cite{lozano2004ontometric,acosta2018detecting,unterkalmsteiner2023compendium,amith2018assessing,yu2015learning,gao2023automatic,watts1998collective}。
前者虽能精确评估具体概念关系，但忽视了taxonomy的整体性和系统性；后者虽能捕捉宏观结构特征，却无法反映构成这一整体的具体概念关系的质量。
这种二元对立的评估范式难以全面把握taxonomy的复杂性。
实际上，有效的taxonomy评估应当在关注细节的同时，能够从微观扩展至宏观，因为taxonomy不仅包含大量概念，更重要的是这些概念之间存在多维度的关系网络，包括垂直层级关系和水平语义关联\cite{Jiang2022TaxoEnrich:}。

评估这种复杂结构的整体质量需要同时考虑多个维度：结构一致性、语义连贯性和层级合理性。此外，由于不同应用场景对taxonomy结构的要求各异，如何将taxonomy的结构精确对齐具体的应用需求也成为一个亟待解决的问题\cite{Liu2024An}。这种多维度、多目标的评估需求大大增加了评估的复杂性和难度。

近年来，大型语言模型（LLMs）的快速发展为解决这些复杂评估问题提供了新的可能。通过在大规模语料上的训练，LLMs展现出了强大的语言理解和知识表征能力，能够很好地理解复杂的结构~\cite{gu2024structext}、语义~\cite{gu2024xiezhi,huang2023c}和上下文信息~\cite{openai2023gpt4}。
这些特性使得LLMs有潜力同时处理taxonomy评估中的微观和宏观问题，并能够灵活适应不同的应用需求\cite{Raiaan2024A}。

然而，直接应用LLMs进行taxonomy评估仍面临着一些挑战。首先，LLMs的输出对输入的微小变化高度敏感，这可能导致评估结果的不稳定性，特别是在评估迭代中的taxonomy时，可能出现不公平或不一致的现象。其次，LLMs的计算效率问题在大规模taxonomy评估中尤为突出。对于包含数十万节点的大型taxonomy，每次迭代后重新评估所有节点将带来巨大的计算开销\cite{Upadhyay2024LLMs}。

鉴于LLMs在taxonomy评估中的潜力和挑战，开发一种能够充分利用LLMs优势，同时克服其局限性的评估框架变得尤为重要。这样的框架不仅需要保证评估的全面性和准确性，还需要考虑评估的效率和一致性。通过合理设计的评估策略和优化技术，有望实现对大规模、复杂taxonomy的高效、公平且全面的评估，从而推动taxonomy在各领域的应用和发展。





==> latex/sections/02.Method.00.tex <==
\subsection{\methode framework}
For effective evaluation of the Taxonomy of the tree structure, our evaluation process is carefully designed into three main steps to ensure the accuracy, efficiency and fairness of the evaluation results. Here is a detailed expansion of each step:
\subsubsection{Step 1: Selection of subtrees}
Our evaluation process starts from the root node of the tree, adopts the top-down breadth-first traversal strategy, gradually deepens the structure of the tree, and selects the eligible subtrees. The core of this step is to find a balance between the quality of the evaluation and the efficiency of the evaluation. In order to reduce the token overhead required by the model during the evaluation process, we pay special attention to the number of nodes in the subtree, ensuring that they are located within a specific interval. This interval is set based on the average output and tree height of the tree, and we set the range as $[average\_output * tree\_height * k, average\_output * tree\_height * 2]$. This method enables us to effectively screen out representative subtree samples and lay a solid foundation for subsequent evaluation. The specific implementation details of the algorithm, such as the selection of traversal algorithm and the calculation method of the number of nodes, are described in detail in \ref{alg:select}.


\subsubsection{Step 2: Calculate the score}
After the subtree is successfully selected, we feed it as a prompt into a pre-trained language model (LLM) to compute a set of predefined score metrics. The design of these indicators is crucial because they are directly related to the explanatory power and application value of the assessment results. In this step, we place particular emphasis on the fairness of the assessment. Since the output of the LLM has a certain randomness, we must ensure that each subtree is evaluated under the same criteria and conditions to eliminate any possible evaluation bias. To this end, we implemented a series of processing methods, including standardizing input formats, using cross-validation techniques, and ensuring consistency of model parameters. Specifically, we effectively control the output of the model by refining the scoring rules, narrowing the range of scores, and requiring the model to output results in a standardized format. In addition, we also adjust the node order of each layer of the tree, change the selection possibility of the subtree, and carry out multiple rounds of cross-validation to enhance the reliability of the evaluation results.

\subsubsection{Step 3: Handling extreme situations}
During the evaluation process, we may encounter some extreme subtree cases that may negatively affect the accuracy of the evaluation results. In order to properly deal with these special cases, we set an explicit interval for the number of nodes in the subtree selection process [A, B]. For example, for a tree with an average output of 10 and a tree height of 5, we might select [50, 100] nodes as a subtree. If the number of children of A parent node exceeds the upper limit B, or falls below the lower limit A, we will impose a penalty on the subtree. The specific way of punishment is to adjust the score of the subtree through a penalty formula to reflect the possible impact of its abnormal node distribution on the evaluation result.
When the number of nodes in the subtree exceeds the set upper limit, the penalty formula is:
$$P = -\lambda * max(1, count/threshold\_high)$$,
when the number of nodes in the subtree is lower than the set lower limit, the penalty formula is: 
$$P = -\mu * max(1, threshold\_low/count)$$, 
where: $P$ represents the penalty fraction, $\lambda$ is a positive penalty coefficient, $\mu$ is another positive penalty coefficient, $count$ is the number of nodes in the subtree, $threshold\_high$ is the upper threshold of the number of nodes, and $threshold\_low$ is the lower threshold of the number of nodes.

\subsection{Metrics}
In order to meet the actual usage needs of Taxonomy, we proposed a series of metrics to prepare for the evaluation. The metrics are as follows:
% hypernyms和hyponyms的定义
\begin{itemize}
    \item \textbf{Single Concept Accuracy (SCA)}: SCA is used to evaluate whether the concepts in Taxomony are clear, concise, and easy to understand as concepts. For example, for the concepts \textit{"FOS prebiotics"} and \textit{"certain prebiotics"}, \textit{"certain prebiotics"} is not as suitable as \textit{"FOS prebiotics"} as a concept word. 
    \item \textbf{Hierarchical Relationship Rationality (HRR)}: HRR is used to evaluate whether the logical hierarchy of hypernyms and hyponyms is appropriate, including whether there are no hyponyms beyond the scope of the hypernym, whether the inclusion relationship is logical, and whether the Hierarchical relationship can be correctly summarized from the examples. If the relationship between the hypernym and hyponym is completely reversed, there is an obvious contradiction or error, such as \textit{"apple"} contains \textit{"fruit"}, then the HRR score should be low.
    \item \textbf{Hierarchical Relationship Exclusiveness (HRE)}:HRE evaluates whether the hypernym can clearly differentiate the list of hyponyms from other unrelated concepts and is sufficiently exclusive. For instance, consider \textit{"product"} and \textbf{"object"} as potential hypernyms for the list \textit{["dairy products", "beauty cosmetics"]}. \textit{"Product"} can more precisely distinguish \textit{"dairy products"} and \textit{"beauty cosmetics"} from other unrelated concepts, whereas \textit{"object"} is too broad and lacks the necessary exclusivity.
    \item \textbf{Hierarchical Relationship Independence (HRI)}: HRI determines the degree of conceptual overlap in a list of hyponyms. For example,  \textit{["citrus fruits", "orange", "grapefruit"]}, where "citrus fruits" contains "orange", which is the concept in the same level, this indicates that some concepts in the subordinate lists are unique while others overlap.
\end{itemize}
